Enabling High Performance Debugging for Variational Quantum Algorithms using Compressed Sensing

Variational quantum algorithms (VQAs) can potentially solve practical problems using contemporary Noisy Intermediate Scale Quantum (NISQ) computers. VQAs find near-optimal solutions in the presence of qubit errors by classically optimizing a loss function computed by parameterized quantum circuits. However, developing and testing VQAs is challenging due to the limited availability of quantum hardware, their high error rates, and the significant overhead of classical simulations. Furthermore, VQA researchers must pick the right initialization for circuit parameters, utilize suitable classical optimizer configurations, and deploy appropriate error mitigation methods. Unfortunately, these tasks are done in an ad-hoc manner today, as there are no software tools to configure and tune the VQA hyperparameters. In this paper, we present OSCAR (cOmpressed Sensing based Cost lAndscape Reconstruction) to help configure: 1) correct initialization, 2) noise mitigation techniques, and 3) classical optimizers to maximize the quality of the solution on NISQ hardware. OSCAR enables efficient debugging and performance tuning by providing users with the loss function landscape without running thousands of quantum circuits as required by the grid search. Using OSCAR, we can accurately reconstruct the complete cost landscape with up to 100X speedup. Furthermore, OSCAR can compute an optimizer function query in an instant by interpolating a computed landscape, thus enabling the trial run of a VQA configuration with considerably reduced overhead.

==> sections/11Rebuttal.tex <==

% \clearpage
\section*{APPENDIX- Revision Summary}
We thank the reviewers for their insightful comments and feedback. We mark all changes in blue. 

\vspace{0.1in}


{\noindent \textbf{Architectural novelty}}
\begin{itemize}
    \item 
\end{itemize}

\vspace{0.05in}

{\noindent \textbf{MainQ2}}
\begin{itemize}
    \item 
    \item 
    \item 
    \item  
\end{itemize}

\vspace{0.05in}


{\noindent \textbf{MainQ3}}
\begin{itemize}
    \item  
\end{itemize}




% The applicability of CS depends on the symmetry of the cost function, i.e. problem Hamiltonian. 
% Common symmetry involves permutation symmetry 
% (variable permutations leave the objective function invariant 
% \cite{shaydulin_classical_2021}),
% Hamiltonian symmetry (led by properties of 
% quantum many-body system in quantum chemistry \cite{lyu_symmetry_2022,ryabinkin_symmetry_2018,seki_symmetry-adapted_2020}), graph symmetry
% (automorphism of a graph \cite{shaydulin_exploiting_2021}), etc.

% Symmetry preserves probability amplitudes,
% i.e., outcomes are invariant under some symmetry group \cite{meyer_exploiting_2022,larocca_group-invariant_2022}.
% Such invariance leads to the symmetry of the landscape,
% where few points are enough to represent the whole landscape.
% This sparsity aligns with the conditions to apply CS.

% % Symmetries are commonly captured by groups and analyzed
% % by representation theory.

% \cite{shaydulin_exploiting_2021} found a connection between classical symmetries of the objective function and the symmetries of the terms of the cost Hamiltonian with respect to the QAOA energy;
% what's more, it shows that 
% such \textbf{symmetry is general and includes
% but is not limited to problems defined on graphs}. 

% \textbf{\cite{fontana_efficient_2022} used spectral analysis to prove that correlated parameter (i.e. correlation led by symmetry) cost functions are efficiently recoverable by CS}. 

% % Symmetry leads to sparsity in the frequency domain, where few points are enough to represent the whole landscape, aligning with the conditions to apply CS.

% Symmetries have already been widely studied in QAOA, VQE, QML, etc. 

% % \textbf{For MaxCut}, \cite{shaydulin_classical_2021} shows that a small set of graph symmetry properties, such as the size of the group of automorphisms of the graph, number of vertex orbits, entropy, etc, suffices to predict the minimum QAOA depth required to achieve a target approximation ratio on \textbf{294 MaxCut graphs with 13 types}.

% \textbf{For VQE}, there is a lot of symmetry due to the correlation of molecules. \cite{lyu_symmetry_2022,ryabinkin_symmetry_2018,seki_symmetry-adapted_2020}
% leverage symmetry of the many-body systems to improve VQE
% in circuit design, state preparation, resource demand, etc.
% We also reconstruct VQE landscapes of H2, LiH, …, N2 by CS in \TODOKUN{Section XX}.

% \textbf{For real quantum device}, the result of reconstruction is shown in \TODOKUN{Section XX}.

% \textbf{For QML}, \cite{meyer_exploiting_2022,larocca_group-invariant_2022,nguyen_theory_2022} explored symmetry groups of the learning problem and dataset to construct models with outcomes invariant under the symmetry of the learning task.

% \textbf{For quantum error mitigation}, 
% \cite{kakkar_characterizing_2022,shaydulin_error_2021,mcardle_error-mitigated_2019,bonet-monroig_low-cost_2018,streif_quantum_2021}
% leverage symmetry of the problems, involving QAOA and VQE, to discover the symmetries of the cost function broken by noise and mitigate them. 

% % Symmetry of a hamiltonian 



% According to [2], symmetry of the problem leads to the symmetry of the cost function; then the symmetry of the cost function leads to the symmetry of Hamiltonian, and thus the QAOA landscapes. Symmetry indicates that in the frequency domain, few points are enough to represent the landscape. This is where CS functions: utilizing the sparsity in the frequency domain to reconstruct the landscape.





==> sections/6ucase-2.tex <==
\newpage

\section{Use Case: Initializing VQAs using OSCAR}
\TODOKUN{rewrite this section}

One common scene is to choose a proper optimizer.
We reconstruct the landscape,
and choose proper optimizer hyperparameters based
on the characteristics and features of the landscape.
E.g. if the landscape is full of salt and pepper noise,
then gradient-free optimizer might be better than gradient-based.

Also, we could perform an optimization on the reconstructed landscape
to precheck the performance,
as shown in Figure \ref{fig:choose_optimizer},
where optimizer B converges while optimizer A fails.
With full landscape in hand, it is natural to think whether
we could perform optimization directly on reconstructed landscape,
instead of on landscape generated directly by VQC.




We find that gradient-free optimizers tends to
give out more available and stable results,
while gradient-based optimizers do not.
But both of them do not perform better than actual QAOA.


% \begin{figure}[h]
% \centering
% \includegraphics[width=\linewidth]{ADAM_optimizer.png}
% \caption{ADAM, gradient-based optimizer.}
% \label{fig:ADAM_optimizer}
% \end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=\linewidth]{Figures/compare_ADAM_and_SPSA.pdf}
% \caption{Optimize on the reconstructed mitigated landscapes with
% interpolation.
% \TODOKUN{replace with n16 version}}
% \label{fig:compare_ADAM_and_SPSA}
% \end{figure}

1. initial point (black)
2. converged point (same one, star)
3. optimal point (color, try, red)
4. path (purple)

iteration for x; cost value for y;

Figure \ref{fig:SPSA_optimizer} and Figure \ref{fig:ADAM_optimizer}
are visualization of optimizations with SPSA and ADAM
on the same 8 qubits, 3-regular MaxCut problem.
For gradient-based optimizer, like ADAM, failed to find the gradient descend path, as shown in sub-figures in the left column
in Figure \ref{fig:ADAM_optimizer}.

There are two theories we propose to explain the difference.
First, noise tends to have an "averaging effect" and makes the landscape
smoother, while mitigation methods will try to break this smoothness. Second, since during optimization, we interpolate points
not lying on the grid. Numerical gradient tends to have large error,
while gradient-free methods do not rely on gradient.

There might be another way to utilize CS as an initialization method.
First, we perform optimization on reconstructed unmitigated landscape
to find a good enough initial point;
next, apply error mitigation techniques and launch the real QAOA optimization \cite{fontana_efficient_2022}.



% {\noindent\textbf{Configure correct initialization:}}

% \begin{figure}[htp]
% \centering
% \includesvg[width=\linewidth]{Figures/choose_initial_point.svg}
% \caption{Configure noise mitigation techniques.}
% \label{fig:choose_initial_point}
% \end{figure}


% One use case of configuring initial points
% is displayed in Figure \ref{fig:choose_initial_point}.
% First, we use CS to reconstruct the landscape.
% Then we choose initial points which are not at barren plateaus
% by naked eye after visualization,
% or numerically choose points which have low cost function value
% on the reconstructed landscape. What's more, we could precheck
% the performance by optimizing on the reconstructed landscape.





==> sections/7Evaluation.tex <==
\section{Evaluation}

% \subsection{Evaluation}

The very first thing to evaluate compressed sensing
is the quality of reconstruction.
According to theory of compressed sensing, sampling rate,
which indicates how much information you obtain directly from
the original signal, matters most.
We define reconstruction accuracy as NCC
between full landscape and reconstructed landscape.
We draw the figure with x-axis as sampling fraction,
y-axis as NCC,
three lines of that under noiseless, unmitigated, and mitigate cases,
as shown in Fig. \ref{fig:compare_optimization}.

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{NCC_vs_sampling_frac.png}
\caption{NCC v.s. sampling fraction.
\TODOKUN{Just an example. To be revised.}
}
\label{fig:compare_optimization}
\end{figure}

\begin{figure}[htp]
\centering
\includegraphics[width=\linewidth]{compare_optimization.png}
\caption{Compare optimization
\TODOKUN{Just an example from other papers. To be changed to ours.}
}
\label{fig:compare_optimization}
\end{figure}

% We compare optimization on full, downsampled and reconstructed landscapes,
% as shown in Fig. \ref{fig:compare_optimization}.

% \TODOKUN{figure}



% Then, we need to verify that $\nopt$ could reflect hardness. 
% We calculate approximate ratio (AR) before and after
% error mitigation.
% We found that $\Delta \nopt$ and AR
% has high correlation value around 0.44,
% verifying that we could take $\Delta\nopt$ has a hardness feature.
% \TODOKUN{figure}
